Absorption of planar massless scalar waves by Kerr black holes

We consider planar massless scalar waves impinging upon a Kerr black hole, for general angles of incidence. We compute the absorption cross section via the partial wave approach, and present a gallery of results. In the low-frequency regime, we show that the cross section approaches the horizon area; in the high-frequency regime, we show that the cross section approaches the geodesic capture cross section. In the aligned case, we extend the complex angular momentum method to obtain a `sinc' approximation, which relates the regular high-frequency oscillations in the cross section to the properties of the polar null orbit. In the non-aligned case, we show, via a semi-analytic approximation, that the reduction in symmetry generates a richer, less regular absorption cross section. We separate the absorption cross section into corotating and counterrotating contributions, showing that the absorption is larger for counterrotating waves, as expected.

==> absorption_kerr_bh.bbl.tex <==
%merlin.mbs apsrev4-1.bst 2010-07-25 4.21a (PWD, AO, DPC) hacked
%Control: key (0)
%Control: author (8) initials jnrlst
%Control: editor formatted (1) identically to author
%Control: production of article title (-1) disabled
%Control: page (0) single
%Control: year (1) truncated
%Control: production of eprint (0) enabled
\begin{thebibliography}{47}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{http://dx.doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Chandrasekhar}(1983)}]{chandra}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Chandrasekhar}},\ }\href@noop {} {\emph {\bibinfo {title} {{Mathematical
  Theory of Black Holes}}}}\ (\bibinfo  {publisher} {Oxford University},\
  \bibinfo {address} {Oxford},\ \bibinfo {year} {1983})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wald}(1984)}]{wald}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Wald}},\ }\href@noop {} {\emph {\bibinfo {title} {{General Relativity}}}}\
  (\bibinfo  {publisher} {The University of Chicago Press},\ \bibinfo {address}
  {Chicago},\ \bibinfo {year} {1984})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chru\'sciel}\ \emph {et~al.}(2012)\citenamefont
  {Chru\'sciel}, \citenamefont {Costa},\ and\ \citenamefont
  {Heusler}}]{lrr-2012-7}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.~T.}\ \bibnamefont
  {Chru\'sciel}}, \bibinfo {author} {\bibfnamefont {J.~L.}\ \bibnamefont
  {Costa}}, \ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Heusler}},\ }\href {\doibase 10.12942/lrr-2012-7} {\bibfield  {journal}
  {\bibinfo  {journal} {Living Reviews in Relativity}\ }\textbf {\bibinfo
  {volume} {15}} (\bibinfo {year} {2012}),\ 10.12942/lrr-2012-7}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Narayan}(2005)}]{Narayan:2005ie}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Narayan}},\ }\href {\doibase 10.1088/1367-2630/7/1/199} {\bibfield
  {journal} {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo {volume}
  {7}},\ \bibinfo {pages} {199} (\bibinfo {year} {2005})},\ \Eprint
  {http://arxiv.org/abs/gr-qc/0506078} {arXiv:gr-qc/0506078 [gr-qc]}
  \BibitemShut {NoStop}%
%%CITATION = GR-QC/0506078;%%
\bibitem [{\citenamefont {Ferrarese}\ and\ \citenamefont
  {Ford}(2005)}]{Ferrarese:2004qr}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Ferrarese}}\ and\ \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Ford}},\ }\href {\doibase 10.1007/s11214-005-3947-6} {\bibfield  {journal}
  {\bibinfo  {journal} {Space Sci. Rev.}\ }\textbf {\bibinfo {volume} {116}},\
  \bibinfo {pages} {523} (\bibinfo {year} {2005})},\ \Eprint
  {http://arxiv.org/abs/astro-ph/0411247} {arXiv:astro-ph/0411247 [astro-ph]}
  \BibitemShut {NoStop}%
%%CITATION = ASTRO-PH/0411247;%%
\bibitem [{\citenamefont {Berti}\ \emph {et~al.}(2009)\citenamefont {Berti},
  \citenamefont {Cardoso},\ and\ \citenamefont {Starinets}}]{berti}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Berti}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Cardoso}}, \
  and\ \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Starinets}},\ }\href
  {\doibase 10.1088/0264-9381/26/16/163001} {\bibfield  {journal} {\bibinfo
  {journal} {Classical Quantum Gravity}\ }\textbf {\bibinfo {volume} {26}},\
  \bibinfo {pages} {163001} (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Risaliti}\ \emph {et~al.}(2013)\citenamefont
  {Risaliti}, \citenamefont {Harrison}, \citenamefont {Madsen}, \citenamefont
  {Walton}, \citenamefont {Boggs}, \citenamefont {Christensen}, \citenamefont
  {Craig}, \citenamefont {Grefenstette}, \citenamefont {Hailey}, \citenamefont
  {Nardini}, \citenamefont {Stern},\ and\ \citenamefont
  {Zhang}}]{Risaliti:2013cga}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Risaliti}}, \bibinfo {author} {\bibfnamefont {F.~A.}\ \bibnamefont
  {Harrison}}, \bibinfo {author} {\bibfnamefont {K.~K.}\ \bibnamefont
  {Madsen}}, \bibinfo {author} {\bibfnamefont {D.~J.}\ \bibnamefont {Walton}},
  \bibinfo {author} {\bibfnamefont {S.~E.}\ \bibnamefont {Boggs}}, \bibinfo
  {author} {\bibfnamefont {F.~E.}\ \bibnamefont {Christensen}}, \bibinfo
  {author} {\bibfnamefont {W.~W.}\ \bibnamefont {Craig}}, \bibinfo {author}
  {\bibfnamefont {B.~W.}\ \bibnamefont {Grefenstette}}, \bibinfo {author}
  {\bibfnamefont {C.~J.}\ \bibnamefont {Hailey}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Nardini}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Stern}}, \ and\ \bibinfo {author} {\bibfnamefont {W.~W.}\
  \bibnamefont {Zhang}},\ }\href {\doibase 10.1038/nature11938} {\bibfield
  {journal} {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo {volume} {494}},\
  \bibinfo {pages} {449} (\bibinfo {year} {2013})},\ \Eprint
  {http://arxiv.org/abs/1302.7002} {arXiv:1302.7002 [astro-ph.HE]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1302.7002;%%
\bibitem [{\citenamefont {Kerr}(1963)}]{kerr}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~P.}\ \bibnamefont
  {Kerr}},\ }\href {\doibase 10.1103/PhysRevLett.11.237} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {11}},\
  \bibinfo {pages} {237} (\bibinfo {year} {1963})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Clifton}\ \emph {et~al.}(2012)\citenamefont
  {Clifton}, \citenamefont {Ferreira}, \citenamefont {Padilla},\ and\
  \citenamefont {Skordis}}]{Clifton:2011jh}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Clifton}}, \bibinfo {author} {\bibfnamefont {P.~G.}\ \bibnamefont
  {Ferreira}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Padilla}}, \
  and\ \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Skordis}},\ }\href
  {\doibase 10.1016/j.physrep.2012.01.001} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rept.}\ }\textbf {\bibinfo {volume} {513}},\ \bibinfo
  {pages} {1} (\bibinfo {year} {2012})},\ \Eprint
  {http://arxiv.org/abs/1106.2476} {arXiv:1106.2476 [astro-ph.CO]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1106.2476;%%
\bibitem [{\citenamefont {Kleihaus}\ \emph {et~al.}(2011)\citenamefont
  {Kleihaus}, \citenamefont {Kunz},\ and\ \citenamefont
  {Radu}}]{Kleihaus:2011tg}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Kleihaus}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Kunz}}, \
  and\ \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Radu}},\ }\href
  {\doibase 10.1103/PhysRevLett.106.151104} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {106}},\ \bibinfo
  {pages} {151104} (\bibinfo {year} {2011})},\ \Eprint
  {http://arxiv.org/abs/1101.2868} {arXiv:1101.2868 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1101.2868;%%
\bibitem [{\citenamefont {Pani}\ \emph {et~al.}(2011)\citenamefont {Pani},
  \citenamefont {Macedo}, \citenamefont {Crispino},\ and\ \citenamefont
  {Cardoso}}]{Pani:2011gy}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Pani}}, \bibinfo {author} {\bibfnamefont {C.~F.}\ \bibnamefont {Macedo}},
  \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Crispino}}, \ and\
  \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Cardoso}},\ }\href
  {\doibase 10.1103/PhysRevD.84.087501} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {84}},\ \bibinfo
  {pages} {087501} (\bibinfo {year} {2011})},\ \Eprint
  {http://arxiv.org/abs/1109.3996} {arXiv:1109.3996 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1109.3996;%%
\bibitem [{\citenamefont {Yagi}\ \emph {et~al.}(2012)\citenamefont {Yagi},
  \citenamefont {Yunes},\ and\ \citenamefont {Tanaka}}]{Yagi:2012ya}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Yagi}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Yunes}}, \ and\
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Tanaka}},\ }\href
  {\doibase 10.1103/PhysRevD.86.044037} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {86}},\ \bibinfo
  {pages} {044037} (\bibinfo {year} {2012})},\ \Eprint
  {http://arxiv.org/abs/1206.6130} {arXiv:1206.6130 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1206.6130;%%
\bibitem [{\citenamefont {Arvanitaki}\ \emph {et~al.}(2010)\citenamefont
  {Arvanitaki}, \citenamefont {Dimopoulos}, \citenamefont {Dubovsky},
  \citenamefont {Kaloper},\ and\ \citenamefont
  {March-Russell}}]{Arvanitaki:2009fg}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Arvanitaki}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Dimopoulos}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Dubovsky}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Kaloper}}, \
  and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {March-Russell}},\
  }\href {\doibase 10.1103/PhysRevD.81.123530} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {81}},\ \bibinfo
  {pages} {123530} (\bibinfo {year} {2010})},\ \Eprint
  {http://arxiv.org/abs/0905.4720} {arXiv:0905.4720 [hep-th]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:0905.4720;%%
\bibitem [{\citenamefont {Arvanitaki}\ and\ \citenamefont
  {Dubovsky}(2011)}]{Arvanitaki:2010sy}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Arvanitaki}}\ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Dubovsky}},\ }\href {\doibase 10.1103/PhysRevD.83.044026} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {83}},\ \bibinfo {pages} {044026} (\bibinfo {year} {2011})},\ \Eprint
  {http://arxiv.org/abs/1004.3558} {arXiv:1004.3558 [hep-th]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1004.3558;%%
\bibitem [{\citenamefont {Boehm}\ and\ \citenamefont
  {Fayet}(2004)}]{Boehm:2003hm}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Boehm}}\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Fayet}},\
  }\href {\doibase 10.1016/j.nuclphysb.2004.01.015} {\bibfield  {journal}
  {\bibinfo  {journal} {Nucl. Phys. B}\ }\textbf {\bibinfo {volume} {683}},\
  \bibinfo {pages} {219} (\bibinfo {year} {2004})},\ \Eprint
  {http://arxiv.org/abs/hep-ph/0305261} {arXiv:hep-ph/0305261 [hep-ph]}
  \BibitemShut {NoStop}%
%%CITATION = HEP-PH/0305261;%%
\bibitem [{\citenamefont {Aad}\ \emph {et~al.}(2012)\citenamefont {Aad} \emph
  {et~al.}}]{Higgs:2012gk}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Aad}} \emph {et~al.} (\bibinfo {collaboration} {ATLAS Collaboration}),\
  }\href {\doibase 10.1016/j.physletb.2012.08.020} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Lett. B}\ }\textbf {\bibinfo {volume} {716}},\
  \bibinfo {pages} {1} (\bibinfo {year} {2012})},\ \Eprint
  {http://arxiv.org/abs/1207.7214} {arXiv:1207.7214 [hep-ex]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1207.7214;%%
\bibitem [{\citenamefont {Crispino}\ \emph
  {et~al.}(2009{\natexlab{a}})\citenamefont {Crispino}, \citenamefont {Dolan},\
  and\ \citenamefont {Oliveira}}]{Crispino:2009xt}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}, \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Dolan}},
  \ and\ \bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont {Oliveira}},\
  }\href {\doibase 10.1103/PhysRevLett.102.231103} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {102}},\
  \bibinfo {pages} {231103} (\bibinfo {year} {2009}{\natexlab{a}})},\ \Eprint
  {http://arxiv.org/abs/0905.3339} {arXiv:0905.3339 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:0905.3339;%%
\bibitem [{\citenamefont {Fabbri}(1975)}]{Fabbri:1975sa}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Fabbri}},\ }\href {\doibase 10.1103/PhysRevD.12.933} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {12}},\
  \bibinfo {pages} {933} (\bibinfo {year} {1975})}\BibitemShut {NoStop}%
%%CITATION = PHRVA,D12,933;%%
\bibitem [{\citenamefont {Sanchez}(1978)}]{Sanchez:1977si}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.~G.}\ \bibnamefont
  {Sanchez}},\ }\href {\doibase 10.1103/PhysRevD.18.1030} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev.D}\ }\textbf {\bibinfo {volume} {18}},\
  \bibinfo {pages} {1030} (\bibinfo {year} {1978})}\BibitemShut {NoStop}%
%%CITATION = PHRVA,D18,1030;%%
\bibitem [{\citenamefont {Gubser}(1997)}]{Gubser:1997cm}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~S.}\ \bibnamefont
  {Gubser}},\ }\href {\doibase 10.1103/PhysRevD.56.7854} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {56}},\
  \bibinfo {pages} {7854} (\bibinfo {year} {1997})},\ \Eprint
  {http://arxiv.org/abs/hep-th/9706100} {arXiv:hep-th/9706100 [hep-th]}
  \BibitemShut {NoStop}%
%%CITATION = HEP-TH/9706100;%%
\bibitem [{\citenamefont {Doran}\ \emph {et~al.}(2005)\citenamefont {Doran},
  \citenamefont {Lasenby}, \citenamefont {Dolan},\ and\ \citenamefont
  {Hinder}}]{Doran:2005vm}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Doran}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Lasenby}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Dolan}}, \ and\ \bibinfo
  {author} {\bibfnamefont {I.}~\bibnamefont {Hinder}},\ }\href {\doibase
  10.1103/PhysRevD.71.124020} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. D}\ }\textbf {\bibinfo {volume} {71}},\ \bibinfo {pages} {124020}
  (\bibinfo {year} {2005})},\ \Eprint {http://arxiv.org/abs/gr-qc/0503019}
  {arXiv:gr-qc/0503019 [gr-qc]} \BibitemShut {NoStop}%
%%CITATION = GR-QC/0503019;%%
\bibitem [{\citenamefont {Crispino}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Crispino}, \citenamefont
  {Oliveira}, \citenamefont {Higuchi},\ and\ \citenamefont
  {Matsas}}]{Crispino:2007qw}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}, \bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont
  {Oliveira}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Higuchi}}, \
  and\ \bibinfo {author} {\bibfnamefont {G.~E.}\ \bibnamefont {Matsas}},\
  }\href {\doibase 10.1103/PhysRevD.75.104012} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo
  {pages} {104012} (\bibinfo {year} {2007}{\natexlab{a}})}\BibitemShut
  {NoStop}%
%%CITATION = PHRVA,D75,104012;%%
\bibitem [{\citenamefont {Jung}\ and\ \citenamefont
  {Park}(2005)}]{Jung:2005mr}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Jung}}\ and\ \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Park}},\
  }\href {\doibase 10.1016/j.nuclphysb.2005.03.037} {\bibfield  {journal}
  {\bibinfo  {journal} {Nucl. Phys. B}\ }\textbf {\bibinfo {volume} {717}},\
  \bibinfo {pages} {272} (\bibinfo {year} {2005})},\ \Eprint
  {http://arxiv.org/abs/hep-th/0502002} {arXiv:hep-th/0502002 [hep-th]}
  \BibitemShut {NoStop}%
%%CITATION = HEP-TH/0502002;%%
\bibitem [{\citenamefont {Crispino}\ \emph
  {et~al.}(2009{\natexlab{b}})\citenamefont {Crispino}, \citenamefont {Dolan},\
  and\ \citenamefont {Oliveira}}]{Crispino:2009ki}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}, \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Dolan}},
  \ and\ \bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont {Oliveira}},\
  }\href {\doibase 10.1103/PhysRevD.79.064022} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {79}},\ \bibinfo
  {pages} {064022} (\bibinfo {year} {2009}{\natexlab{b}})},\ \Eprint
  {http://arxiv.org/abs/0904.0999} {arXiv:0904.0999 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:0904.0999;%%
\bibitem [{\citenamefont {Crispino}\ and\ \citenamefont
  {Oliveira}(2008)}]{Crispino:2008zz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}\ and\ \bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont
  {Oliveira}},\ }\href {\doibase 10.1103/PhysRevD.78.024011} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {78}},\ \bibinfo {pages} {024011} (\bibinfo {year} {2008})}\BibitemShut
  {NoStop}%
%%CITATION = PHRVA,D78,024011;%%
\bibitem [{\citenamefont {Oliveira}\ \emph {et~al.}(2011)\citenamefont
  {Oliveira}, \citenamefont {Crispino},\ and\ \citenamefont
  {Higuchi}}]{Oliveira:2011zz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont
  {Oliveira}}, \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}, \ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Higuchi}},\ }\href {\doibase 10.1103/PhysRevD.84.084048} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {84}},\ \bibinfo {pages} {084048} (\bibinfo {year} {2011})}\BibitemShut
  {NoStop}%
%%CITATION = PHRVA,D84,084048;%%
\bibitem [{\citenamefont {Glampedakis}\ and\ \citenamefont
  {Andersson}(2001)}]{Glampedakis:2001cx}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Glampedakis}}\ and\ \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Andersson}},\ }\href {\doibase 10.1088/0264-9381/18/10/309} {\bibfield
  {journal} {\bibinfo  {journal} {Classical Quantum Gravity}\ }\textbf
  {\bibinfo {volume} {18}},\ \bibinfo {pages} {1939} (\bibinfo {year}
  {2001})},\ \Eprint {http://arxiv.org/abs/gr-qc/0102100} {arXiv:gr-qc/0102100
  [gr-qc]} \BibitemShut {NoStop}%
%%CITATION = GR-QC/0102100;%%
\bibitem [{\citenamefont {Dolan}(2006)}]{dolanthesis}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Dolan}},\ }\emph {\bibinfo {title} {Scattering, absorption and emission by
  black holes}},\ \href@noop {} {Ph.D. thesis},\ \bibinfo  {school} {Trinity
  Hall and Astrophysics Group, Cavendish Laboratory, University of Cambridge},
  \bibinfo {address} {Cambridge, England} (\bibinfo {year} {2006})\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Dolan}(2008)}]{Dolan:2008kf}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont
  {Dolan}},\ }\href {\doibase 10.1088/0264-9381/25/23/235002} {\bibfield
  {journal} {\bibinfo  {journal} {Classical Quantum Gravity}\ }\textbf
  {\bibinfo {volume} {25}},\ \bibinfo {pages} {235002} (\bibinfo {year}
  {2008})},\ \Eprint {http://arxiv.org/abs/0801.3805} {arXiv:0801.3805 [gr-qc]}
  \BibitemShut {NoStop}%
%%CITATION = ARXIV:0801.3805;%%
\bibitem [{\citenamefont {Crispino}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Crispino}, \citenamefont
  {Oliveira},\ and\ \citenamefont {Matsas}}]{Crispino:2007zz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}, \bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont
  {Oliveira}}, \ and\ \bibinfo {author} {\bibfnamefont {G.~E.}\ \bibnamefont
  {Matsas}},\ }\href {\doibase 10.1103/PhysRevD.76.107502} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {107502} (\bibinfo {year}
  {2007}{\natexlab{b}})}\BibitemShut {NoStop}%
%%CITATION = PHRVA,D76,107502;%%
\bibitem [{\citenamefont {Dolan}\ \emph {et~al.}(2009)\citenamefont {Dolan},
  \citenamefont {Oliveira},\ and\ \citenamefont {Crispino}}]{Dolan:2009zza}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont
  {Dolan}}, \bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont {Oliveira}},
  \ and\ \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Crispino}},\
  }\href {\doibase 10.1103/PhysRevD.79.064014} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {79}},\ \bibinfo
  {pages} {064014} (\bibinfo {year} {2009})},\ \Eprint
  {http://arxiv.org/abs/0904.0010} {arXiv:0904.0010 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:0904.0010;%%
\bibitem [{\citenamefont {Dolan}\ \emph {et~al.}(2012)\citenamefont {Dolan},
  \citenamefont {Oliveira},\ and\ \citenamefont {Crispino}}]{Dolan:2011ti}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont
  {Dolan}}, \bibinfo {author} {\bibfnamefont {L.~A.}\ \bibnamefont {Oliveira}},
  \ and\ \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Crispino}},\
  }\href {\doibase 10.1103/PhysRevD.85.044031} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {85}},\ \bibinfo
  {pages} {044031} (\bibinfo {year} {2012})},\ \Eprint
  {http://arxiv.org/abs/1105.1795} {arXiv:1105.1795 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1105.1795;%%
\bibitem [{\citenamefont {Oliveira}\ \emph {et~al.}(2010)\citenamefont
  {Oliveira}, \citenamefont {Dolan},\ and\ \citenamefont
  {Crispino}}]{Oliveira:2010zzb}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.~S.}\ \bibnamefont
  {Oliveira}}, \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Dolan}},
  \ and\ \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Crispino}},\
  }\href {\doibase 10.1103/PhysRevD.81.124013} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {81}},\ \bibinfo
  {pages} {124013} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
%%CITATION = PHRVA,D81,124013;%%
\bibitem [{cai()}]{caio_erratum}%
  \BibitemOpen
  \href@noop {} {}\bibinfo {note} {We would like to take the opportunity to
  point out a misprint in Ref. \cite{Macedo:2012zz}, where a factor of
  $\sin^2\theta$ is missing in the $g_{\varphi\varphi}$ component of the Kerr
  metric. This misprint does not affect any other expression or result in Ref.
  \cite{Macedo:2012zz}.}\BibitemShut {Stop}%
	
	\bibitem [{\citenamefont {Macedo}\ \emph {et~al.}(2012)\citenamefont {Macedo},
  \citenamefont {Crispino},\ and\ \citenamefont {Cardoso}}]{Macedo:2012zz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~F.}\ \bibnamefont
  {Macedo}}, \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont
  {Crispino}}, \ and\ \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont
  {Cardoso}},\ }\href {\doibase 10.1103/PhysRevD.86.024002} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {86}},\ \bibinfo {pages} {024002} (\bibinfo {year} {2012})}\BibitemShut
  {NoStop}%

\bibitem [{\citenamefont {Carter}(1968)}]{carter}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Carter}},\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal}
  {Commun. Math. Phys.}\ }\textbf {\bibinfo {volume} {10}},\ \bibinfo {pages}
  {280} (\bibinfo {year} {1968})}\BibitemShut {NoStop}%
%%CITATION = CMPHA,10,280;%%
\bibitem [{\citenamefont {Brill}\ \emph {et~al.}(1972)\citenamefont {Brill},
  \citenamefont {Chrzanowski}, \citenamefont {Martin~Pereira}, \citenamefont
  {Fackerell},\ and\ \citenamefont {Ipser}}]{brill}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Brill}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Chrzanowski}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Martin~Pereira}},
  \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Fackerell}}, \ and\
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Ipser}},\ }\href
  {\doibase 10.1103/PhysRevD.5.1913} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {5}},\ \bibinfo {pages} {1913}
  (\bibinfo {year} {1972})}\BibitemShut {NoStop}%
%%CITATION = PHRVA,D5,1913;%%
\bibitem [{\citenamefont {Flammer}(1957)}]{spheroid}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont
  {Flammer}},\ }\href@noop {} {\emph {\bibinfo {title} {{Spheroidal Wave
  Functions}}}}\ (\bibinfo  {publisher} {Stanford University Press},\ \bibinfo
  {address} {Stanford},\ \bibinfo {year} {1957})\BibitemShut {NoStop}%
%%CITATION = PHRVA,D86,024002;%%
\bibitem [{\citenamefont {Ottewill}\ and\ \citenamefont
  {Winstanley}(2000)}]{Ottewill:2000qh}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~C.}\ \bibnamefont
  {Ottewill}}\ and\ \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Winstanley}},\ }\href {\doibase 10.1103/PhysRevD.62.084018} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume}
  {62}},\ \bibinfo {pages} {084018} (\bibinfo {year} {2000})},\ \Eprint
  {http://arxiv.org/abs/gr-qc/0004022} {arXiv:gr-qc/0004022 [gr-qc]}
  \BibitemShut {NoStop}%
%%CITATION = GR-QC/0004022;%%
\bibitem [{\citenamefont {Press}\ and\ \citenamefont
  {Teukolsky}(1972)}]{Press:1972zz}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {W.~H.}\ \bibnamefont
  {Press}}\ and\ \bibinfo {author} {\bibfnamefont {S.~A.}\ \bibnamefont
  {Teukolsky}},\ }\href {\doibase 10.1038/238211a0} {\bibfield  {journal}
  {\bibinfo  {journal} {Nature}\ }\textbf {\bibinfo {volume} {238}},\ \bibinfo
  {pages} {211} (\bibinfo {year} {1972})}\BibitemShut {NoStop}%
%%CITATION = NATUA,238,211;%%
\bibitem [{\citenamefont {Higuchi}(2001)}]{Higuchi:2001si}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Higuchi}},\ }\href {\doibase 10.1088/0264-9381/18/20/102} {\bibfield
  {journal} {\bibinfo  {journal} {Classical Quantum Gravity}\ }\textbf
  {\bibinfo {volume} {18}},\ \bibinfo {pages} {L139} (\bibinfo {year}
  {2001})},\ \bibinfo {note} {\textbf{19}, 599 (2002)},\ \Eprint
  {http://arxiv.org/abs/hep-th/0108144} {arXiv:hep-th/0108144 [hep-th]}
  \BibitemShut {NoStop}%
%%CITAx'TION = HEP-TH/0108144;%%
\bibitem [{\citenamefont {Zakharov}\ \emph {et~al.}(2005)\citenamefont
  {Zakharov}, \citenamefont {Nucita}, \citenamefont {DePaolis},\ and\
  \citenamefont {Ingrosso}}]{Zakharov:2005nb}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Zakharov}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Nucita}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {DePaolis}}, \ and\
  \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Ingrosso}},\ }\href@noop
  {} {\  (\bibinfo {year} {2005})},\ \Eprint
  {http://arxiv.org/abs/gr-qc/0507118} {arXiv:gr-qc/0507118 [gr-qc]}
  \BibitemShut {NoStop}%
%%CITATION = GR-QC/0507118;%%
\bibitem [{\citenamefont {D\'ecanini}\ \emph
  {et~al.}(2011{\natexlab{a}})\citenamefont {D\'ecanini}, \citenamefont
  {Esposito-Far\`ese},\ and\ \citenamefont {Folacci}}]{DEFF}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {D\'ecanini}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Esposito-Far\`ese}}, \ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Folacci}},\ }\href {\doibase 10.1103/PhysRevD.83.044032}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo
  {volume} {83}},\ \bibinfo {pages} {044032} (\bibinfo {year}
  {2011}{\natexlab{a}})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {D\'ecanini}\ \emph
  {et~al.}(2011{\natexlab{b}})\citenamefont {D\'ecanini}, \citenamefont
  {Folacci},\ and\ \citenamefont {Raffaelli}}]{DFR}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont
  {D\'ecanini}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Folacci}},
  \ and\ \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Raffaelli}},\
  }\href {\doibase 10.1088/0264-9381/28/17/175021} {\bibfield  {journal}
  {\bibinfo  {journal} {Class.Quant.Grav.}\ }\textbf {\bibinfo {volume} {28}},\
  \bibinfo {pages} {175021} (\bibinfo {year} {2011}{\natexlab{b}})},\ \Eprint
  {http://arxiv.org/abs/1104.3285} {arXiv:1104.3285 [gr-qc]} \BibitemShut
  {NoStop}%
%%CITATION = ARXIV:1104.3285;%%
\bibitem [{\citenamefont {Yang}\ \emph {et~al.}(2012)\citenamefont {Yang},
  \citenamefont {Nichols}, \citenamefont {Zhang}, \citenamefont {Zimmerman},
  \citenamefont {Zhang},\ and\ \citenamefont {Chen}}]{Yang:2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont
  {Yang}}, \bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont {Nichols}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Zhang}}, \bibinfo
  {author} {\bibfnamefont {A.}~\bibnamefont {Zimmerman}}, \bibinfo {author}
  {\bibfnamefont {Z.}~\bibnamefont {Zhang}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {Chen}},\ }\href {\doibase
  10.1103/PhysRevD.86.104006} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. D}\ }\textbf {\bibinfo {volume} {86}},\ \bibinfo {pages} {104006}
  (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dolan}(2010)}]{Dolan:2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont
  {Dolan}},\ }\href {\doibase 10.1103/PhysRevD.82.104003} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. D}\ }\textbf {\bibinfo {volume} {82}},\
  \bibinfo {pages} {104003} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ford}\ and\ \citenamefont
  {Wheeler}(1959)}]{Ford1959287}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {K.~W.}\ \bibnamefont
  {Ford}}\ and\ \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont
  {Wheeler}},\ }\href {\doibase 10.1016/0003-4916(59)90027-2} {\bibfield
  {journal} {\bibinfo  {journal} {Ann. Phys.}\ }\textbf {\bibinfo {volume}
  {7}},\ \bibinfo {pages} {287 } (\bibinfo {year} {1959})}\BibitemShut
  {NoStop}%
\end{thebibliography}%

